Predictive Multiplicity in Classification

Prediction problems often admit competing models that perform almost equally well. This effect challenges key assumptions in machine learning when competing models assign conflicting predictions. In this paper, we define predictive multiplicity as the ability of a prediction problem to admit competing models with conflicting predictions. We introduce formal measures to evaluate the severity of predictive multiplicity and develop integer programming tools to compute them exactly for linear classification problems. We apply our tools to measure predictive multiplicity in recidivism prediction problems. Our results show that real-world datasets may admit competing models that assign wildly conflicting predictions, and motivate the need to measure and report predictive multiplicity in model development.

==> figure/baseline_summary.tex <==
\begin{tabular}{lcc}
\toprule
                         \bfcell{c}{Dataset} & 
                         \bfcell{c}{Training\\Error} & 
                         \bfcell{c}{Test\\Error} \\
\midrule
         \textds{compas\_arrest} &        32.7\% &      33.4\% \\
        \textds{compas\_violent} &        37.7\% &       37.9\%\\
   \textds{pretrial\_CA\_arrest} &        34.1\%  &       34.4\%  \\
      \textds{pretrial\_CA\_fta} &        36.3\% &      36.3\% \\
   \textds{pretrial\_NY\_arrest} &        27.8\% &      39.7\% \\
      \textds{pretrial\_NY\_fta} &        25.9\%&      29.9\% \\
 \textds{recidivism\_CA\_arrest} &        34.4\% &      34.2\% \\
   \textds{recidivism\_CA\_drug} &        36.3\% &      36.2\% \\
 \textds{recidivism\_NY\_arrest} &        31.0\% &      31.8\% \\
   \textds{recidivism\_NY\_drug} &        32.5\% &      33.6\% \\
\bottomrule
\end{tabular}


==> figure/compas_arrest_01_comparison_table.tex <==
\begin{tabular}{llll}
\toprule
model type         &                               baseline &                               discrepancy &                               flipped \\
Score Function     &  \coeftbl{compas_arrest}{01}{baseline} &  \coeftbl{compas_arrest}{01}{discrepancy} &  \coeftbl{compas_arrest}{01}{flipped} \\
$h(\xb_i)$         &                                    + 1 &                                       - 1 &                                   - 1 \\
$score(\xb_i)$     &                                  + 3.5 &                                     - 0.2 &                                 - 0.1 \\
discrepancy train  &                                    0.0 &                                      17.4 &                                   5.4 \\
discrepancy test   &                                    0.0 &                                      17.5 &                                   6.2 \\
error train        &                                   32.1 &                                      33.1 &                                  32.1 \\
error test         &                                   35.7 &                                      34.5 &                                  35.0 \\
\bottomrule
\end{tabular}


==> figure/compas_arrest_01_model_baseline.tex <==
\begin{tabular}{@{\;}c@{\;}r@{\,}l@{\;}c@{\;}r@{\,}l@{\;}c@{\;}r@{\,}l}
 $-$ &   7.0 &                  \textfn{race$=$causasian} &  $+$ &  3.6 &          \textfn{race$=$african\_american} &  $-$ &   2.3 &                   \textfn{race$=$hispanic} \\
 $+$ &   0.0 &                      \textfn{race$=$other} &  $+$ &  9.5 &                       \textfn{age$\leq$25} &  $+$ &   0.0 &                        \textfn{age\_25-45} \\
 $-$ &   8.2 &                       \textfn{age$\geq$46} &  $-$ &  7.0 &                            \textfn{female} &  $-$ &   3.4 &                     \textfn{n\_priors$=$0} \\
 $+$ &   0.0 &                  \textfn{n\_priors$\geq$1} &  $+$ &  8.2 &                  \textfn{n\_priors$\geq$2} &  $+$ &  12.9 &                  \textfn{n\_priors$\geq$5} \\
 $-$ &   3.7 &     \textfn{n\_juvenile\_misdemeanors$=$0} &  $+$ &  3.4 &  \textfn{n\_juvenile\_misdemeanors$\geq$1} &  $-$ &   2.3 &  \textfn{n\_juvenile\_misdemeanors$\geq$2} \\
 $-$ &  24.8 &  \textfn{n\_juvenile\_misdemeanors$\geq$5} &  $+$ &  0.0 &         \textfn{n\_juvenile\_felonies$=$0} &  $+$ &   1.2 &      \textfn{n\_juvenile\_felonies$\geq$1} \\
 $+$ &   0.0 &      \textfn{n\_juvenile\_felonies$\geq$2} &  $+$ &  0.0 &      \textfn{n\_juvenile\_felonies$\geq$5} &  $-$ &   2.3 &                \textfn{charge\_degree$=$M} \\
 $+$ &   0.0 &                                            &      &      &                                            &      &       &                                            \\
\end{tabular}


==> figure/compas_arrest_01_model_discrepancy.tex <==
\begin{tabular}{@{\;}c@{\;}r@{\,}l@{\;}c@{\;}r@{\,}l@{\;}c@{\;}r@{\,}l}
 $+$ &   0.4 &                  \textfn{race$=$causasian} &  $+$ &   0.0 &          \textfn{race$=$african\_american} &  $-$ &   0.5 &                   \textfn{race$=$hispanic} \\
 $+$ &   0.2 &                      \textfn{race$=$other} &  $+$ &   0.0 &                       \textfn{age$\leq$25} &  $-$ &   0.5 &                        \textfn{age\_25-45} \\
 $-$ &  20.2 &                       \textfn{age$\geq$46} &  $-$ &  19.4 &                            \textfn{female} &  $-$ &   0.4 &                     \textfn{n\_priors$=$0} \\
 $+$ &   0.0 &                  \textfn{n\_priors$\geq$1} &  $+$ &  19.3 &                  \textfn{n\_priors$\geq$2} &  $+$ &  19.7 &                  \textfn{n\_priors$\geq$5} \\
 $+$ &   0.3 &     \textfn{n\_juvenile\_misdemeanors$=$0} &  $+$ &   0.0 &  \textfn{n\_juvenile\_misdemeanors$\geq$1} &  $+$ &   0.0 &  \textfn{n\_juvenile\_misdemeanors$\geq$2} \\
 $+$ &   0.0 &  \textfn{n\_juvenile\_misdemeanors$\geq$5} &  $+$ &   0.0 &         \textfn{n\_juvenile\_felonies$=$0} &  $+$ &  18.9 &      \textfn{n\_juvenile\_felonies$\geq$1} \\
 $+$ &   0.0 &      \textfn{n\_juvenile\_felonies$\geq$2} &  $+$ &   0.0 &      \textfn{n\_juvenile\_felonies$\geq$5} &  $+$ &   0.2 &                \textfn{charge\_degree$=$M} \\
 $+$ &   0.0 &                                            &      &       &                                            &      &       &                                            \\
\end{tabular}


==> figure/compas_arrest_01_model_flipped.tex <==
\begin{tabular}{@{\;}c@{\;}r@{\,}l@{\;}c@{\;}r@{\,}l@{\;}c@{\;}r@{\,}l}
 $-$ &  1.2 &                  \textfn{race$=$causasian} &  $+$ &   0.0 &          \textfn{race$=$african\_american} &  $-$ &  1.0 &                   \textfn{race$=$hispanic} \\
 $-$ &  0.8 &                      \textfn{race$=$other} &  $+$ &   1.3 &                       \textfn{age$\leq$25} &  $+$ &  0.0 &                        \textfn{age\_25-45} \\
 $-$ &  1.9 &                       \textfn{age$\geq$46} &  $-$ &   0.5 &                            \textfn{female} &  $+$ &  0.0 &                     \textfn{n\_priors$=$0} \\
 $-$ &  0.2 &                  \textfn{n\_priors$\geq$1} &  $+$ &   2.1 &                  \textfn{n\_priors$\geq$2} &  $+$ &  2.0 &                  \textfn{n\_priors$\geq$5} \\
 $+$ &  0.0 &     \textfn{n\_juvenile\_misdemeanors$=$0} &  $+$ &   0.4 &  \textfn{n\_juvenile\_misdemeanors$\geq$1} &  $-$ &  0.9 &  \textfn{n\_juvenile\_misdemeanors$\geq$2} \\
 $-$ &  2.7 &  \textfn{n\_juvenile\_misdemeanors$\geq$5} &  $-$ &   0.4 &         \textfn{n\_juvenile\_felonies$=$0} &  $+$ &  0.0 &      \textfn{n\_juvenile\_felonies$\geq$1} \\
 $-$ &  0.8 &      \textfn{n\_juvenile\_felonies$\geq$2} &  $+$ &  82.8 &      \textfn{n\_juvenile\_felonies$\geq$5} &  $-$ &  0.8 &                \textfn{charge\_degree$=$M} \\
 $+$ &  0.0 &                                            &      &       &                                            &      &      &                                            \\
\end{tabular}


==> figure/workshop_compas_arrest_small_01_comparison_table.tex <==
\begin{tabular}{lccc}
\toprule
&
\bfcell{c}{Baseline\\Model} &
\bfcell{c}{Individual Ambiguity\\Model} &
\bfcell{c}{Discrepancy\\Model} \\

\toprule

$h(\xb_p)$  &                                           $+1$ &    
    $-$1 &
    $-$1 \\

\toprule

Error (Train)        &                                         32.7\% &                                            32.7\% &                                        33.6\%\\
Error (Test)         &                                         33.4\% &                                            33.4\% &                                        34.5\% \\

\toprule

Discrepancy (Train)  &                                          0.0\% &                                            0.0037\% &                                      16.8\% \\ %3.7e-02\% \\
Discrepancy (Test)   &                                          0.0\% &                                            0.0\% &                                         15.1\% \\

% \toprule
% \cell{l}{Score\\Function}     &  
% \coeftbl{compas_arrest_small}{01}{baseline} &  
% \coeftbl{compas_arrest_small}{01}{flipped} &
% \coeftbl{compas_arrest_small}{01}{discrepancy} \\

%\toprule


%$s(\xb_p)$     &                                        16.1 &                                            $-$0.1 &                                       $-$0.5 \\

\bottomrule
\end{tabular}


==> tyranny_table.tex <==

\begin{table}[h]
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{ll}
\toprule
\bfcell{l}{Notation} & \bfcell{l}{Description} \\
\toprule 
$\xb_i \in \R^{d+1}$ & feature vector 
\\ \midrule
$y_i \in \{-1, +1\}$ & class label 
\\ \midrule
$\truerisk{\cdot}$ & true risk (Bayes' error)
\\ \midrule
$\emprisk{\cdot}$ & empirical risk (training error)
\\ \midrule
$\bestclf{}$ & most accurate classifier
\\ \midrule
$\altclf{i}$ & most accurate classifier s.t. $\altclf{i}(\xb_i) = -\bestclf{}(\xb_i)$
\\ \midrule 
$\diffclf{\epsilon}$ & most different classifier in the $\epsilon$-level set of $\bestclf{}$ \\ 
\bottomrule
\end{tabular}
}
\caption{Table of Notation}
\label{Table:Notation}
\end{table}

\subsection*{Toy Examples}

\begin{figure}[t]
\centering
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{c*{3}{>{\hspace{0.5em}}rrc}}
& \multicolumn{3}{c}{\textsc{Group A}}
& \multicolumn{3}{c}{\textsc{Group B}}
& \multicolumn{3}{c}{\textsc{Pooled}} \\ 
\cmidrule(lr){2-4} 
\cmidrule(lr){5-7} 
\cmidrule(lr){8-10}

$(x_1, x_2)$ &  
$\nplus{}$ & $\nminus{}$ & ${h^*_A}$ & 
$\nplus{}$ & $\nminus{}$ & ${h^*_B}$ &
$\nplus{}$ & $\nminus{}$ & $\bestclf{}$ \\ 

\cmidrule(lr){1-1} 
\cmidrule(lr){2-4} 
\cmidrule(lr){5-7} 
\cmidrule(lr){8-10}

(0, 0) & 
50 & 101 & - &
100 & 50 & + &
150 & 151 & - \\ 

(0, 1) & 
101 & 50 & + &
50 & 100 & - &
151 & 150 & + \\ 

(1, 0) & 
101 & 50 & + &
50 & 100 & - &
151 & 150 & + \\ 

(1, 1) & 
101 & 50 & + &
50 & 100 & - &
151 & 150 & + \\ 

\cmidrule(lr){1-1} 
\cmidrule(lr){2-4} 
\cmidrule(lr){5-7} 
\cmidrule(lr){8-10}
\end{tabular}
}
\caption{We are given data from two groups $z \in \{ A, B\}$ with heterogeneous data distributions $\prob{y = + 1 | \xb, A} = \prob{y = -1 |\xb, B}$. Here, $\nplus{}$ and $\nminus{}$ denote the number of training examples with $y = +1$ and $y = -1$. }
\label{Fig::TyrannyOfMajority}
\end{figure}

